Likelihood-based inference and forecasting for trawl processes: a stochastic optimization approach

We consider trawl processes, which are stationary and infinitely divisible stochastic processes and can describe a wide range of statistical properties, such as heavy tails and long memory. In this paper, we develop the first likelihood-based methodology for the inference of real-valued trawl processes and introduce novel deterministic and probabilistic forecasting methods. Being non-Markovian, with a highly intractable likelihood function, trawl processes require the use of composite likelihood functions to parsimoniously capture their statistical properties. We formulate the composite likelihood estimation as a stochastic optimization problem for which it is feasible to implement iterative gradient descent methods. We derive novel gradient estimators with variances that are reduced by several orders of magnitude. We analyze both the theoretical properties and practical implementation details of these estimators and release a Python library which can be used to fit a large class of trawl processes. In a simulation study, we demonstrate that our estimators outperform the generalized method of moments estimators in terms of both parameter estimation error and out-of-sample forecasting error. Finally, we formalize a stochastic chain rule for our gradient estimators. We apply the new theory to trawl processes and provide a unified likelihood-based methodology for the inference of both real-valued and integer-valued trawl processes.

==> introduction_old.tex <==
\input{notation}
\newpage
\textbf{To be done later:}
\begin{itemize}
\item choosing the parameterizations for the VG distribution for Appendix \ref{appendix:parameterizations and reparameterizations}, as well as in any other part of the paper where these distributions appear. 
\item bibliography: some of the citations have bad formatting, will fix at the end
\end{itemize}
\textbf{Other questions to be discussed during the meeting}
\begin{itemize}
\item titles for Figures 2 and 3; add text? might be very long. too short as it is? 
\item Figure 4: do we need a simulation study for the bias and variance reduction, or just the densities are good enough?
\item questions about the introduction:
%\item displaying the forecast results. idea 1, simulation-based: we get a time series of losses for each of GMM and CL for each simulation. do we do a t-test on the mean/median-losses? or do we just display the ratio of mean/median losses? idea 2, KL and Wasserstein based: in Gaussian and KL we can compute the KL divergence *** of the predictable part of the error, for NIG we can only compute the W distance for all the errors in \eqref{eq:implicit_grad}, $\epsilon$ is the variable I use as the argument for the density of the unif. distr. on $[0,1]$, which is clearly not the same as a random sample from the unif. distr. Would it be clearer if I removed the part: 'where $\epsilon$ is a random sample from the unif. distr.'? is there a risk of confusion between $\mathcal{N}(0,1)$ and $\mathcal{U}(0,1)$ as base distributions which don t depend on $\bt$ in the remaining of the subsection?
\item Simulation results before practical implementation details so i can refer back to the figures, although it s switching back and forth.
    \item difficulties maintaining the list of notations with the new notations for Figures \ref{fig:grads_whole_fig}, \ref{fig:likelihood_cv_whole_fig}, \ref{fig:grads_cv_whole_fig} 
\end{itemize}
\newpage


==> notation.tex <==
\newpage
\textbf{Notation: OLD PLEASE IGNORE THIS PAGE}
\begin{itemize}
\item $\bt$ parameters of the L\'evy seed and acf
    \item $n$ number of translations of the trawl set, i.e. the 'length' of the discretely observed path $X_{\tau},\ldots,X_{n\tau}$.
    \item $\textrm{Distribution\_Name}(x;\bt)$ is the pdf. example: $\mathcal{N}(x;\mu,\sigma^2)$ and $\textrm{Gamma}(x;\alpha,\beta)$  are pdfs
    \item  the joint likelihood $l(\bt;x_t,x_s) = p(x_t,x_s;\bt)$ is often written  as $l(\bt)$, where the dependency on the fixed realisations of $x_t,x_s$ of the trawl process is implicit 
    \item $l(\bt) = p(x_t,x_s;\bt)$ can be written $\ev_{q(z;\bt)}[f(z,\bt)]$ where $q$ is the distribution of $L(A)$ for some set $A$, a truncation of $L(A)$ or another distribution if the expression for the joint likelihood simplifies. $f$ also depends on $x_t,x_s$. when there is no risk of confusion, we drop $x_t,x_s$ from the notation $l(\bt)$ 
    \item $\nabla_{\bt}z$ pathwise gradient of a sample from $q(\cdot;\bt)$ with respect to $\bt$ given by $\frac{\nabla_{\bt}F(z;\bt)}{p(z;\bt)}$. $\nabla_{\bt}Z$ is defined similarly.
    \item $U_i = f(Z_i)$ and $V_i = \nabla_{\bt} f(Z_i,\bt) + \pdv{f}{z}(Z_i,\bt) \nabla_{\bt} Z_i $, where $Z_i$ are iid with law $q(\cdot;\bt)$. Then $U_i$, $V_i$ are consistent, unbiased estimators for $l(\bt) = \ev_{q(z;\bt)}[f(z,\bt)]$ and respectively for $\nabla_{\bt}\ev_{q(z;\bt)}[f(z,\bt)] = \ev_{q(z;\bt)}[f(z,\bt) + \pdv{f}{z} \nabla_{\bt} z ]$. Then the log likelihood $\log{p(x_t,x_s;\bt)} $ is estimated by $\log{\left(\frac{U_1 + ... U_n}{n}\right)}$ and its gradient w.r.t $\bt$ is estimated by $\frac{V_1+\ldots+V_n}{U_1 + \ldots+U_n}.$
        \item $m$ degree of the taylor polynomial to be used in control variates 
    \item $\gamma$ and $\gamma_i$ for $i=0,1,2,3$ are optimal for the control variate method
    \item $u(x_t,x_s;\bt) \defeq \Var{(U_i)} = \Var{\left(f(Z_i)\right)}$, $u_{m}(x_t,x_s;\bt) \defeq \Var{(U_i - \gamma T_f)} = \Var{\left(f(Z_i) - \gamma T_f(Z_i)\right)}$ where $T_f$ is a Taylor polynomial of degree $m$, $u(\bt) = \ev_{p(x_t,x_s;\bt)}[u(x_t,x_s;\bt)]$, $u_m(\bt) = \ev_{p(x_t,x_s;\bt)}[u_m(x_t,x_s;\bt)]$ [add the r.v. formulation]
    \item SF (score function),  PG (patwhise gradient)
    \item $v^{\text{SF}}(x_t,x_s;\bt)$ and  $v^{\text{PG}}(x_t,x_s;\bt)$ are the variance of estimators for $\nabla_{\bt}l(\bt)$. $v^{\text{SF}}_m(\bt) \defeq  \ev_{p(x_t,x_s;\bt)}\left[v^{\text{SF}}(x_t,x_s;\bt)\right] $, $v^{\text{PG}}_m(\bt) \defeq  \ev_{p(x_t,x_s;\bt)}\left[v^{\text{PG}}(x_t,x_s;\bt)\right]$. When the subscript $m$ is added ($ex:$ $v^{\text{SF}}_m$ and $v^{\text{PG}}_m$), we also use CV with a taloy polynomial of degree $m$.
    \item $N$ number of samples in MC estimators
\end{itemize}

==> old_examples.tex <==
\begin{example}[Poisson L\'evy basis]\label{ex:distr_poisson}
Let $L^{'}\sim \text{Poisson}(\nu)$. Then $X_t = L(A_t) \sim \text{Poisson}(\nu\mathrm{Leb}\left(A\right)).$ 
\end{example}
\begin{example}[Negative Binomial L\'evy basis]gsf\label{ex:distr_negbin}
\end{example}
\begin{example}[Skellam L\'evy basis]
Let $L'\sim \text{Skellam}(\mu_1,\mu_2),$ i.e.~$L^{'}\sim N_1 - N_2$ with $N_1,N_2$ independent and Poisson distributed with intensities $\mu_1,\mu_2 >0.$  Then $X_t = L(A_t) \sim \text{Skellam}(\mu_1 \mathrm{Leb}\left(A\right),\mu_2 \mathrm{Leb}\left(A\right)).$\label{ex:distr_skellam}
\end{example}
\begin{example}[Gamma L\'evy basis]\label{ex:distr_gamma}
Let $L^{'} \sim \text{Gamma}(\alpha,\beta)$ with $p(x) = \frac{\beta^\alpha}{\Gamma(\alpha)} x^{\alpha-1} \exp{(-\beta x)}$, $x, \, \alpha, \, \beta>0.$
Then $X_t = L(A_t) \sim \text{Gamma}(\alpha \mathrm{Leb}\left(A\right),\beta).$
\end{example}
\begin{example}[Inverse Gaussian L\'evy basis]\label{ex:distr_ig}
Let $L^{'} \sim \text{IG}(\mu,\lambda)$ with $p(x) = \sqrt{\frac{\lambda}{2 \pi x^3}} \allowbreak \exp \left(-\frac{\lambda(x-\mu)^2}{2 \mu^2 x}\right)$. Then $X_t = L(A_t) \sim \textrm{IG}(\mu \mathrm{Leb}(A),\lambda \mathrm{Leb}^2(A))$.
\end{example}
%\begin{example}[Inverse Gaussian L\'evy basis]\label{ex:distr_ig}
%Let $L^{'} \sim \text{IG}(\delta,\gamma)$ with pdf
% $p(x) = \frac{\delta}{\sqrt{2 \pi x^3}} \exp{\left(\delta \gamma- \frac{\delta^2 + \gamma^2x^2}{2x}\right)}$, $x>0, \, \delta >0, \, \gamma>0.$
%Then $X_t = L(A_t) \sim \textrm{IG}(\delta \mathrm{Leb}\left(A\right),\gamma).$
%\end{example}
\begin{example}[Gaussian L\'evy basis]\label{ex:distr_gaussian}
Let $L^{'}\sim \mathcal{N}(\mu,\sigma^2)$. Then $X_t = L(A_t) \sim \mathcal{N}\left(\mu \mathrm{Leb}\left(A\right), \sigma^2 \mathrm{Leb}\left(A\right)\right).$
\end{example}
An important class of infinitely divisible distributions is that of Normal variance-mean mixtures (see ), which include the following two particular cases.


\begin{tabular}{ |c||c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{Discrete Distributions} \\
 \hline \hline
 Distribution& Range & Parameters & PMF & CF \\
 \hline
$\textrm{Poisson}(\lambda)$ & $ \Z^{+} $   & $\alpha < \beta \in \R$ &   $\frac{\lambda^x e^{-\lambda}}{x!}$ & $\exp{\left(\lambda(e^{it}-1)\right)}$ \\  \hline
 $\textrm{NB}(m,p)$& $\mathbb{Z}^{+}$ &   \begin{tabular}{c} $m \in \R^{+}$ \\$p \in [0,1]$\end{tabular} & & \\ \hline
 $\textrm{Skellam}(\mu_1,\mu_2)$& $\mathbb{Z}$ & $\mu_1, \mu_2 > 0$  & $e^{-(\mu_1+\mu_2)} \left(\frac{\mu_1}{\mu_2}\right)^{x/2} I_{|x|}(2 \sqrt{\mu_1 \mu_2})$ & $exp{\left(-\left(\mu_1+\mu_2\right)+\mu_1 e^{i t}+\mu_2 e^{-i t}\right)}$ \\\hline
\end{tabular}

\begin{tabular}{ |c||c|c|c|c|  }
 \hline
 \multicolumn{5}{|c|}{Continuous Distributions} \\
 \hline \hline
 Distribution& Range & Parameters & PDF & CF \\
 \hline
$\mathcal{U}(\alpha,\beta)  $ & $ (\alpha,\beta) $   & $\alpha < \beta \in \R$ &   $\frac{1}{\beta - \alpha}$ & $\begin{cases}\frac{\mathrm{e}^{i  t \beta}-\mathrm{e}^{i t \alpha}}{i t(\beta-\alpha)} & \text { for } t \neq 0 \\ 1 & \text { for } t=0\end{cases}$ \\  \hline
 $\textrm{Beta}(\alpha,\beta)$ & $(0,1)$ & $\alpha,\beta>0$&  $\frac{x^{\alpha-1}(1-x)^{\beta-1}}{\textrm{B}(\alpha,\beta)}$ & $_{1}F_{1}(\alpha;\alpha + \beta; it) $\\ \hline
  $\textrm{Gamma}(\alpha,\beta)$& $\R^{+}$    & $\alpha, \beta \in \R^{+}$   & $\frac{\beta^\alpha}{\Gamma(\alpha)} x^{\alpha-1} e^{(-\beta x)}$  $\left(1 - \frac{it}{\beta}\right)^{-\alpha} $& \\ \hline
 $\textrm{IG}(\mu,\lambda)$& $\R^{+}$     & $\mu, \lambda \in \R^{+}$ & &\\ \hline
$\mathcal{N}(\mu,\sigma^2)$ & $\R$ & \begin{tabular}{c} $\mu \in \R$ \\$\sigma^2 \in \R^{+}$\end{tabular}
  &  $\frac{1}{\sqrt{2 \pi \sigma^2}}e^{-\left(\frac{x-\mu}{\sigma}\right)^2}$ & $e^{i \mu t - \sigma^2 t^2/2}$\\ \hline
   $\mathcal{M}(\mu,\sigma^2)$ & $\R$& \begin{tabular}{c} $\mu \in \R$ \\$\sigma^2 \in \R^{+}$\end{tabular} & $\frac{1}{\sqrt{2 \pi}} \frac{(x-\mu)^2}{\sigma^3} e^{-\left(\frac{x-\mu}{\sigma}\right)^2}$  & $(1-\sigma^2 t^2) e^{i \mu t - \sigma^2 t^2/2}$\\ \hline
   $\textrm{NIG}(\alpha,\beta,\delta,\mu)$& $\R$  &    &  &\\ \hline %https://www.wolframalpha.com/input?i=Fourier+transform+calculator&assumption=%7B%22F%22%2C+%22FourierTransformCalculator%22%2C+%22transformfunction%22%7D+-%3E%22%28x-mu%29%5E2%2F%28+%282+*+pi+%29%5E0.5+*+sigma%5E3%29+++*+e%5E%7B-%28x-mu%29%5E2%2F+%282*+sigma%5E2%29%7D%22&assumption=%7B%22F%22%2C+%22FourierTransformCalculator%22%2C+%22variable1%22%7D+-%3E%22x%22&assumption=%7B%22F%22%2C+%22FourierTransformCalculator%22%2C+%22variable2%22%7D+-%3E%22t%22
  $\textrm{VG}$&   &    & & \\ \hline
\end{tabular}

==> proofs.tex <==
\section{Proofs}
\label{section_proofs}

We now turn to the proof of Theorem \ref{thm:non_markovian_forecast}, for which we will need the following two results.
%\begin{theorem}[L\'evy-It\^o decomposition of L\'evy bases: adaptation of Theorem 4.5 from \cite{pedersen2003levy}]
%\label{thm:levy_ito_decomp_for_levy_bases}
%Let $L$ be a L\'evy basis on $S \subset \R^d$ with characteristic triplet $(\xi,\,a,\,l)$, where $\xi \in \R,\, a \in \R_{\ge 0}$ and $l$ is a L\'evy measure on $\R$. Let $\nu = \mathrm{Leb} \otimes l$ be the product measure on $S \times \R,$ where $\mathrm{Leb}$ is the Lebesgue measure on $S.$ %i.e. the unique $\simga-\text{finite}$ measure on $B_{\mathrm{Leb}}\left(S \times R\right)$ with $\nu(A \times )$
%Then there exists a decomposition of $L$ into independent L\'evy bases: a Gaussian part $L_g$ with characteristic triplet $(\xi,\,a,\,0)$ and two jump parts $L_j^{+}$ and $L_j^{-}$ with characteristic triplets $(0,\,0,\,l^{+})$ and $(0,\,0,\,l^{-})$, such that for any $A \in B_{\mathrm{Leb}}(S),$ the following holds a.s.
%\begin{equation*}
%    L(A) = L_g(A) + L_j^{+}(A) + L_j^{-}(A),
%\end{equation*}
%where $l^{+}$ and $l^{-}$ are the restrictions of $l$ to the positive and negative real lines.
%Moreover, there exists a Poisson random measure $N$ on $\mathcal{B}_{\mathrm{Leb}} (S)\times \R$ with intensity measure $\nu$ such that
%\begin{equation*}
%    L_j\left(A\right) = \int_A \int_{(-1,1)} y \ \mathrm{d} (N- \nu)(\mathbf{z},y) + \int_A \int_{\R \backslash(-1,1)} y \ \mathrm{d} N(\mathbf{z},y),
    %\label{eq:poisson representation}
%\end{equation*}
%where $\mathbf{z} = (t,\mathbf{x}) \in S$ and $y \in \R$ and  
%\begin{align*}
%    L_g^{+} & \defeq \int_A \int_{(0,1)} y \ \mathrm{d} (N- \nu)(\mathbf{z},y) + \int_A \int_{(1,\infty)} y \ \mathrm{d} N(\mathbf{z},y), \\
%    L_g^{-} & \defeq \int_A \int_{(-1,0)} y \ \mathrm{d} (N- \nu)(\mathbf{z},y) + \int_A \int_{(-\infty,-1)} y \ \mathrm{d} N(\mathbf{z},y)
%\end{align*}.
%\end{theorem}
%The L\'evy bases $L_j^{+}$ and $L_j^{-}$ are only contain the positive, respectively negative jumps of $L_j$.
\begin{lemma}
\label{lemma:exchangeable}
Let $Y_1,\ldots,Y_n $ be integrable and exchangeable real-valued random variables. Then 
\begin{equation*}
    \ev[Y_1|Y_1 + \ldots + Y_n] = \frac{Y_1 + \ldots + Y_n}{n}. 
\end{equation*}
\end{lemma}
\begin{proof}[Proof of Theorem \ref{thm:non_markovian_forecast}]
By the independence of $L(A_t)$ and $L(A_{t+h}\backslash A_t)$, we have that
\begin{align*}
\ev[X_{t+h} | X_t] =& \ev[L(A_{t+h}\cap A_t) | L(A_t)] + \ev[L( A_{t+h} \backslash A_t)| L(A_t)]\\ =& \ev[L(A_{t+h}\cap A_t) | L(A_t)] + \ev[L( A_{t+h} \backslash A_t)] \\
=& \ev[L(A_{t+h} \cap A_t) | L(A_t)] + \frac{Leb(A_h\backslash A)}{Leb(A)} \ev[X_t].
\end{align*}
hence it is enough to prove that
\begin{equation}\label{eq:conditional_it_is_enough}
    \ev[L( A_{t+h} \cap A_t) | L(A_t)] = \frac{Leb(A_h\cap A)}{Leb(A)} X_t.
\end{equation}
We prove relation  \eqref{eq:conditional_it_is_enough} by analysing two cases.

\underline{Case I:} If $\frac{Leb(A \backslash A_h)}{Leb(A_h \cap A)}= \frac{m}{n} \in \mathbb{Q}$ for some positive integers $m$ and $n$, let
\begin{equation*}
   q \defeq \frac{Leb(A \backslash A_h)}{m} = \frac{Leb(A_h \cap A)}{n}.
\end{equation*}
and partition $A \backslash A_h$ into $m$ disjoint subsets $S_1,\ldots,S_n$ of area $q$ and $A \cap A_h$ into $n$ disjoint subsets $S_{n+1},\ldots,S_{n+m}$ of area $q.$ Then $L(S_1),\ldots,L(S_{n+m})$ are iid and integrable and by Lemma \ref{lemma:exchangeable}, we obtain that
\begin{align*}
    \ev\left[L(A_{t+h}\cap A_t)|L(A_t)\right] =& \sum_{j=1}^n \ev\left[ L(S_j) \bigg\rvert \sum_{i=1}^{n+m} L(S_i)\right]\\ =& \frac{n}{n+m} \sum_{i=1}^{n+m} L(S_i) = \frac{Leb(A_h \cap A)}{Leb(A)} L(A_t).
\end{align*} 
\underline{Case II:} If $\frac{Leb(A \backslash A_h)}{Leb(A_h \cap A)}= \alpha \not\in \mathbb{Q}$ let $\alpha_n \in \mathbb{Q}$ with $\alpha_n \uparrow \alpha.$ Consider a nested sequences of sets $A_t \cap A_{t+h} \subset   \ldots   \subset S_{n+1} \subset S_n \ldots \subset S_1 \subset A_t$ such that
\begin{equation*}
\bigcap_{n} S_n = A_t \cap A_{t+h} \ \textrm{  and  } \ \frac{Leb(A\backslash S_n)}{Leb(S_n)} =  \alpha_n.
\end{equation*}
By the proof of Case I, we have that $    \ev[L(S_n)|L(A_t)] = \frac{Leb(S_n)}{Leb(A)} L(A_t)$.
Since $\frac{Leb(S_n)}{Leb(A)} \to \frac{Leb(A\cap A_h)}{Leb(A)},$ we have that  $\ev[L(S_n)|L(A_t)] \to \frac{Leb(A\cap A_h)}{Leb(A)} L(A_t)$ a.s. By the uniqueness of the limit, it is enough to prove that $L(S_n) \to L(A \cap A_h)$ in $\mathcal{L}^1$, or equivalently $L\left(S_n \backslash (A_h \cap A)\right) \to 0$ in $\mathcal{L}^1$. % $\ev[L(S_n)|L(A_t)] \to \ev[L(A \cap A_h)|L(A_t)],$ or equivalently
%\begin{equation*}
%    \ev\left[L\left(S_n \backslash (A_h \cap A)\right) \big\rvert  L(A_t)\right] \to 0  \textrm{ as } n \to \infty.
%\end{equation*}
%For ease of notation, let $Z_n \defeq S_n \backslash (A_h \cap A)$.
We show that the sequence $L\left(S_n \backslash (A_h \cap A)\right)$ convergence in probability to $0$ and is uniformly integrable.   %We prove the stronger statement that $L\left(Z_n\right) \to 0$ in $\mathcal{L}^1,$ which follows from the fact that the sequence of random variables $L\left(Z_n\right)$ converges to $0$ in probability and is uniformly integrable. 
We have that $\ev\left[e^{i t L\left(S_n \backslash (A_h \cap A)\right)} \right] =  \mathrm{Leb}\left(S_n \backslash (A_h \cap A)\right) \, \ev\left[e^{i t L^{'}} \right] \to 0 $ as $n \to \infty$, hence $L\left(S_n \backslash (A_h \cap A)\right) \to 0$ in distribution, hence in probability. Further, by theorem \ref{thm:levy_ito_decomp_for_levy_bases}, the L\'evy basis $L$ can be decomposed in $L= L_g + L_j^{+} + L_j^{-}$, and since $L^{'}$ is integrable, $L_j^{+}$ and $L_j^{-}$ are also integrable. %By the same argument as above, we get that $L_g(Z_n),\, L_j^{+}(Z_n),\, L_j^{-}(Z_n) \to 0$ as $n \to \infty$ in probability. 
Note that the sequences $L_j^{+}(Z_n)$ and $L_j^{-}(Z_n)$ are integrable, monotonic and dominated by $L_j^{+}(Z_1)$ and $L_j^{-}(Z_1)$, hence uniformly integrable. Finally, note that $L_g(Z_n)$ is uniformly bounded in $\mathcal{L}^2$, hence uniformly integrable. Finally, Thus the sequence $L(Z_n)$ is uniformly integrable.
%For the uniform integrability, note that for fixed $K>0,$ the mapping $
%n \to \ev\left[|Z| 1_{|Z| > K }\right] $ is decreasing, hence
%\begin{equation*}
%    \lim_{K \to \infty} \sup_{n} \ev\left[|Z_n| 1_{|Z_n| > K }\right]  = \lim_{K \to \infty}  \ev\left[|Z_1| 1_{|Z_1| > K }\right] = 0
%\end{equation*}
%by DCT, since $Z_1$ is integrable. [to rewrite proof, we need U.I., which follows by decomposing L into $L_g$, $L_p^{+}$ and $L_p^{-}$]
\end{proof}



==> simulation_study/extra_figures.tex <==
\begin{figure}[H]
 \centering
\subfloat[$\alpha=1,\beta = 2,\lambda = 1$]{\label{}\includegraphics[width=.33\linewidth]{example-image-a}}\hfill
\subfloat[asd]{\label{}\includegraphics[width=.33\linewidth]{example-image-b}}\hfill
\subfloat[asd]{\label{}\includegraphics[width=.33\linewidth]{example-image-c}}\par 
\subfloat[afs]{\label{}\includegraphics[width=.33\linewidth]{example-image-b}}\hfill
\subfloat[sdf]{\label{}\includegraphics[width=.33\linewidth]{example-image-c}}\hfill
\subfloat[s]{\label{}\includegraphics[width=.33\linewidth]{example-image-a}}\par 
\subfloat[s]{\label{}\includegraphics[width=.33\linewidth]{example-image-b}}\hfill
\subfloat[d]{\label{}\includegraphics[width=.33\linewidth]{example-image-b}}\hfill
\subfloat[sim study std red grad lambda title to change]{\label{}\includegraphics[width=.33\linewidth]{example-image-b}}
\caption{inference results for gaussian levy seed}
\label{fig:inference_results_gaussian_levy_seed}
\end{figure}
\begin{figure}[H]
 \centering
\subfloat[$\alpha=1,\beta = 2,\lambda = 1$]{\label{}\includegraphics[width=.33\linewidth]{example-image-a}}\hfill
\subfloat[s]{\label{}\includegraphics[width=.33\linewidth]{example-image-b}}\hfill
\subfloat[a]{\label{}\includegraphics[width=.33\linewidth]{example-image-c}}\par 
\subfloat[s]{\label{}\includegraphics[width=.33\linewidth]{example-image-b}}\hfill
\subfloat[s]{\label{}\includegraphics[width=.33\linewidth]{example-image-c}}\hfill
\subfloat[a]{\label{}\includegraphics[width=.33\linewidth]{example-image-a}}\par 
\subfloat[]{\label{}\includegraphics[width=.33\linewidth]{example-image-b}}\hfill
\subfloat[]{\label{}\includegraphics[width=.33\linewidth]{example-image-b}}\hfill
\subfloat[sim study std red grad lambda title to change]{\label{}\includegraphics[width=.33\linewidth]{example-image-b}}
\caption{inference results for nig levy seed}
\label{fig:inference_results_nig_levy_seed}
\end{figure}


==> supplementary_material/Simple_ambit_field_inference.tex <==
\subsection{Simple ambit fields inference}\label{subsection:simple_ambit_field}
Trawl processes are stationary and infinitely divisible continuous-time stochastic processes which can describe a wide range of possible serial correlation patterns in data. A direct generalization of the trawl process to spatio-temporal fields is given by the ambit field $Y$ with
\begin{equation}
    Y_t(\mathbf{x}) = \int_{A_t(\mathbf{x})} K_{t,\mathbf{x}}\left(\bar{t},\bar{\mathbf{x}}\right) \sigma(\bar{t},\bar{\mathbf{x}}) L(\mathrm{d}\bar{t},\mathrm{d}\bar{\mathbf{x}}),\label{def:ambit_fields}
\end{equation}
where the deterministic kernel $K$ multiplied by the volatility $\sigma$ is integrated against the L\'evy basis $L$ and where $A_t(\mathbf{x}) \in \R^{d+1}$ is a collection of time and space-indexed sets. The integration is understood in the sense of \cite[Theorem 2.7]{rajput1989spectral} when the integrand is determinstic, i.e.~$\sigma = 1$, and in the sense of 
\cite{walsh,bichteler1983random} and \cite{kluppelberg} for stochastic $\sigma$. Ambit fields provide a powerful statistical modelling framework, and we only mention a few examples.  \cite{di2014forecasting} uses Gaussian L\'evy bases to forecast 
energy market contracts and 
\cite{ambit_book} discusses forward curve modelling by ambit fields in Chapter $11$. \cite{emil_h_phd_thesis} provides extensive analyses of turbulence and energy dissipation through  L\'evy modelling and ambit fields and \cite{jonsdottir2008levy} introduces a new approach by ambit fields to growth modelling and applies it to tumour growth. The last two papers use GMM to calibrate the model parameters, which can have poor finite sample performance or be unfeasible for somedistributions (e.g.~see page $15$ of \citep{emil_h_phd_thesis}). \cite{jonsdottir2008levy} introduces non-rectangular ambit sets and non-Gaussian L\'evy bases, extending beyond both the Markovian and Gaussian frameworks for spatio-temporal modelling. This added complexity of the model which helps replicate the stylised statistical facts of the datasets is also the issue with applying these models further. For example, we are not aware of deterministic or probabilistic forecasting formulae for ambit fields, even in the case when $\sigma = 1 $ in \eqref{def:ambit_fields}. To improve on this, we propose the use of simple ambit fields, which we discuss below.

Simple ambit fields are a natural extension of trawl processes to spatio-temporal fields and are given by 
$Y_t(\mathbf{x}) = L(A_t(\mathbf{x}))$. Similarly to trawl processes, simple ambit fields provide a rich class of infinitely divisible stochastic processes with flexible spatio-temporal autocorrelation structures and marginal distributions, which can be modelled independently one of the other. In particular, the autocovariance and autocorrelation structures are 
\begin{align*}
\Cov(Y_{t_1}(\mathbf{x}_1),Y_{t_2}(\mathbf{x}_2)) &=  \mathrm{Leb}\left(A_{t_1}(\mathbf{x})\cap A_{t_2}(\mathbf{x}_2)\right)  \Var(L^{'})\\ \Corr(Y_{t_1}(\mathbf{x}_1),Y_{t_2}(\mathbf{x}_2)) &= \mathrm{Leb}\left((A_{t_1}(\mathbf{x}_1)\cap A_{t_2}(\mathbf{x}_2)\right) / \, {\mathrm{Leb}\left(A\right)} 
 \end{align*}
and $Y$ can have any infinitely divisible distribution. We generally fix an ambit set $A \in \R^{d+1}$ and let $A_t(\mathbf{x}) = A + (t,\mathbf{x})$ be the set translation of $A$. With this choice of ambit sets, $Y$ is stationary and can be simulated efficiently by two algorithms (see Section $5$ of \cite{leonte2022simulation_arxiv}). Further, we show that both the composite likelihood inference and forecasting methodology extends from trawl processes to simple ambit fields, making the latter a tractable approach for spatio-temporal statistics. To begin with, the following conditional mean forecast formula holds.
\begin{theorem}Assume that the L\'evy seed $L^{'}$ is integrable. Then 
\begin{equation*}
    \ev\left[Y_{t+\Delta_t}(\mathbf{x}+ \mathbf{\Delta_x}) | Y_t(\mathbf{x}) \right] = \rho \, Y_t(\mathbf{x}) + (1-\rho) \,\ev[Y_t(\mathbf{x})],
\end{equation*}
where 
\begin{equation*}
\rho\ =  \frac{\mathrm{Leb}\left(A_t(\mathbf{x}) \cap A_{t+\Delta_t}(\mathbf{x} + \mathbf{\Delta_x})\right)}{\mathrm{Leb}(A)}.
\end{equation*}
\end{theorem}
The same proof as for Theorem \ref{thm:non_markovian_forecast} applies and probabilistic sampling can be performed as described in Section \ref{section_forecasting}. We now turn our attention to composite likelihood estimation. For ease of exposition, we present the theory in $d=1$ dimensions.

Let $\tau,\,  x>0$ and assume we observe a realization $\mathbf{y}$ of the simple ambit field $Y$ at time-space coordinates $\{(i\tau,jx): 1 \le i \le n_s, 1 \le j \le n_x\}$. Then $\y$ is $n_s \times n_t$ dimensional. Define the temporal and spatial pairwise likelihood function at lags $k_t$ and $k_s$ by
\begin{align*}
    {PL}_{\textrm{t}}^{k_t}(\bt;\y) &= \prod_{i=1}^{n_t-k_t} 
 \prod_{j=1}^{n_s}p\left(y_{i\tau}(jx),y_{(i+k_t)\tau}(jx);\bt\right),     \\
     {PL}_{\textrm{s}}^{k_s}(\bt;\y)& = \prod_{i=1}^{n_t} 
 \prod_{j=1}^{n_s-k_s}p\left(y_{i\tau}(jx),y_{i\tau}\left((j+k_s)x\right);\bt\right), 
\end{align*}
and the pairwise likelihood function by
\begin{equation*}
\mathcal{L}_{PL}(\bt) =  \prod_{k_t \in K_t} \prod_{k_s \in K_s} {PL}_{\textrm{t}}^{k_t}(\bt;\y)   \, {PL}_{\textrm{s}}^{k_s}(\bt;\y),
\end{equation*}
where $K_t$ and $K_s$ are the numbers of temporal, respectively spatial lags to be included. The PL estimator is then given by
\begin{equation*}
\end{equation*}
\begin{equation*}
    \hat{\bt}^{PL} \defeq \argmax_{\bt} \mathcal{L}_{PL}(\bt).
\end{equation*}
The pairwise likelihoods can be estimated with samples, as described at the beginning of Section \ref{subsection:trawl_inference_as_a_stoch_optim_problem}. The variance reductions techniques presented in Subsections \ref{subsubsection:pg}, \ref{subsubsection_linear_control_variateas} and in S\ref{supplementary:measure_valued_grad}, i.e.~pathwise gradients, measure-value gradients and control variates can be applied directly, with no change. 

[some tables with results to add]

\textbf{Further research}

Firstly, the above composite likelihood inference procedure for simple ambit fields only included pairs corresponding to either vertical or horizontal translations of ambit sets. Given an $n_s \times n_t$ matrix $\y$ of observations, these pairs only account for a fraction of the total number of pairs for which the corresponding ambit sets have non-empty intersection. We expect that using more pairs will result in better finite sample properties of our estimators. The difficulty lies in approximating the areas of the intersections of ambit sets which are translated along both axes of coordinates. A solution would be to work with families of trawl functions $\phi$ for which these areas are available analytically.

Secondly, although composite likelihood proves to be an efficient inference method for simple ambit fields, it can not be applied to ambit fields in general. The presence of the deterministic kernel $K$ or stochastic volatility $\sigma$ in \ref{def:ambit_fields} makes the pairwise likelihood and even the marginal likelihood function intractable. It is not clear if ambit fields are always ergodic and further and even so, GMM is known to perform poorly for certain distributions (e.g.~NIG). This significantly restricts parameter calibration and the applicability of ambit fields to real-world modelling problems. Nevertheless, using ambit fields instead of simple ambit fields has advantages, e.g.~directly modelling non-stationary behaviour by ambit fields rather then fitting simple ambit fields to a de-trended and de-seasonalised dataset, which might be only covariance stationary and not strictly stationary. To this extent, we refer the new advances in the amortized likelihood inference \cite{?} [ a few citations], which use first use neural networks to approximate the likelihood function and then perform MCMC to sample from the posterior distribution of the model parameters. 




